An Empirical Study of Fuzz Harness Degradation

The purpose of continuous fuzzing platforms is to enable fuzzing for software projects via fuzz harnesses -- but as the projects continue to evolve, are these harnesses updated in lockstep, or do they run out of date? If these harnesses remain unmaintained, will they degrade over time in terms of coverage achieved or number of bugs found? This is the subject of our study. We study Google's OSS-Fuzz continuous fuzzing platform containing harnesses for 510 open-source C/C++ projects, many of which are security-critical. A harness is the glue code between the fuzzer and the project, so it needs to adapt to changes in the project. It is often added by a project maintainer or as part of a, sometimes short-lived, testing effort. Our analysis shows a consistent overall fuzzer coverage percentage for projects in OSS-Fuzz and a surprising longevity of the bug-finding capability of harnesses even without explicit updates, as long as they still build. However, we also identify and manually examine individual cases of harness coverage degradation and categorize their root causes. Furthermore, we contribute to OSS-Fuzz and Fuzz Introspector to support metrics to detect harness degradation in OSS-Fuzz projects guided by this research.

==> generated/latex-data.tex <==
\makeatletter\newcommand\data[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\data@out{\PackageError{data}{this is a container: Dict{Symbol, Any}(:cleanedData => Dict(:numCommits => 2556947, :numCrashRevisions => 83863, :numIntrospector => 712094, :numHarnessIntrospector => 929224, :numProjects => 491, :numCoverage => 574840, :numHarnessChanges => 29923, :numCves => 1997, :numMonorailBugs => 53460), :numDegradationWithoutMax => 696, :harnessCutoff => "100", :numBrokenProjects => 28, :lastData => "2024-10", :numInstancesDegradation => 257, :rq1Wilcoxon => Dict{Symbol, Dict{Symbol, LaTeXStrings.LaTeXString}}(:perProjectRelNoOutliers => Dict(:confIntHigh => L"$0.031$", :estimate => L"$0.023$", :pValue => L"1.1 e^{-12}", :confIntLow => L"$0.015$"), :perProjectRel => Dict(:confIntHigh => L"$0.039$", :estimate => L"$0.028$", :pValue => L"1.0 e^{-14}", :confIntLow => L"$0.019$"), :perProjectCov => Dict(:confIntHigh => L"$0.082$", :estimate => L"$0.03$", :pValue => L"0.21", :confIntLow => L"$-0.018$"), :perProjectCovNoOutliers => Dict(:confIntHigh => L"$0.078$", :estimate => L"$0.028$", :pValue => L"0.22", :confIntLow => L"$-0.018$"), :perHarnessRel => Dict(:confIntHigh => L"$0.017$", :estimate => L"$0.013$", :pValue => L"1.1 e^{-20}", :confIntLow => L"$0.01$"), :perHarnessCovNoOutliers => Dict(:confIntHigh => L"$0.013$", :estimate => L"$0.006$", :pValue => L"0.03", :confIntLow => L"$0.001$"), :perHarnessCov => Dict(:confIntHigh => L"$0.009$", :estimate => L"$0.003$", :pValue => L"0.30", :confIntLow => L"$-0.002$"), :perHarnessRelNoOutliers => Dict(:confIntHigh => L"$0.014$", :estimate => L"$0.01$", :pValue => L"2.7 e^{-17}", :confIntLow => L"$0.007$")), :rq1HarnessOutliers => "176", :lastMonorail => "2024-09-11", :numProjectsWithCoverageData => 510, :hurStats => Dict{Symbol, Dict{Symbol, LaTeXStrings.LaTeXString}}(:bugs => Dict(:estimate => L"$0.649$", :pValue => L"2.2 e^{-16}"), :cov => Dict(:estimate => L"$-0.365$", :pValue => L"4.2 e^{-12}")), :filteredData => Dict(:numCommits => 2357857, :numCrashRevisions => 78045, :numIntrospector => 554269, :numHarnessIntrospector => 781749, :numProjects => 342, :numCoverage => 453744, :numHarnessChanges => 9609, :numCves => 1856, :numMonorailBugs => 49020), :numDegradationStudies => 257, :classificationCounts => Dict("entriesLow" => 87, "unknown" => 9, "gcovError" => 6, "total" => 322, "intededHarnessRemoval" => 4, "codeChurn" => 28, "projectCode" => 43, "buildFailure" => 27, "libraryCode" => 47, "entriesDecrease" => 71), :numDoneDegradationStudies => 328, :numProjectsWithCommits => 491, :bootstrapReps => "10,000", :cumsumBuckets => "2,000", :churnCauseCounts => Dict("harnessFail" => 12, "fuzzerRegression" => 4, "revival" => 23, "features" => 29, "other" => 3, "total" => 71), :numIntroHarnesses => 2117, :commitProjs => Dict(:unclean => 491, :removedNotAvailable => 19, :removedClean => 9, :unfiltered => 482), :uncleanData => Dict(:numCommits => 8297824, :numCrashRevisions => 104494, :numIntrospector => 975213, :numHarnessIntrospector => 1307652, :numProjects => 510, :numCoverage => 665165, :numHarnessChanges => 42412, :numCves => 3360, :numMonorailBugs => 68486), :rq1HarnessCount => "6,411", :coverageReportsMissing => "18.14", :earliestOSSProject => "2016-10", :harnessUpdateStats => Dict{Symbol, Real}(:max => 93.0, :min => -85.98, :deviation => 4.48, :mean => 0.25, :count => 6520, :median => 0.0))}{use an element}}\else\ifnum\pdfstrcmp{#1}{cleanedData}=0\let\data@out\data@I\else\ifnum\pdfstrcmp{#1}{numDegradationWithoutMax}=0\def\data@out{$696$}\else\ifnum\pdfstrcmp{#1}{harnessCutoff}=0\def\data@out{100}\else\ifnum\pdfstrcmp{#1}{numBrokenProjects}=0\def\data@out{$28$}\else\ifnum\pdfstrcmp{#1}{lastData}=0\def\data@out{2024-10}\else\ifnum\pdfstrcmp{#1}{numInstancesDegradation}=0\def\data@out{$257$}\else\ifnum\pdfstrcmp{#1}{rq1Wilcoxon}=0\let\data@out\data@II\else\ifnum\pdfstrcmp{#1}{rq1HarnessOutliers}=0\def\data@out{176}\else\ifnum\pdfstrcmp{#1}{lastMonorail}=0\def\data@out{2024-09-11}\else\ifnum\pdfstrcmp{#1}{numProjectsWithCoverageData}=0\def\data@out{$510$}\else\ifnum\pdfstrcmp{#1}{hurStats}=0\let\data@out\data@III\else\ifnum\pdfstrcmp{#1}{filteredData}=0\let\data@out\data@IV\else\ifnum\pdfstrcmp{#1}{numDegradationStudies}=0\def\data@out{$257$}\else\ifnum\pdfstrcmp{#1}{classificationCounts}=0\let\data@out\data@V\else\ifnum\pdfstrcmp{#1}{numDoneDegradationStudies}=0\def\data@out{$328$}\else\ifnum\pdfstrcmp{#1}{numProjectsWithCommits}=0\def\data@out{$491$}\else\ifnum\pdfstrcmp{#1}{bootstrapReps}=0\def\data@out{10,000}\else\ifnum\pdfstrcmp{#1}{cumsumBuckets}=0\def\data@out{2,000}\else\ifnum\pdfstrcmp{#1}{churnCauseCounts}=0\let\data@out\data@VI\else\ifnum\pdfstrcmp{#1}{numIntroHarnesses}=0\def\data@out{$2{,}117$}\else\ifnum\pdfstrcmp{#1}{commitProjs}=0\let\data@out\data@VII\else\ifnum\pdfstrcmp{#1}{uncleanData}=0\let\data@out\data@VIII\else\ifnum\pdfstrcmp{#1}{rq1HarnessCount}=0\def\data@out{6,411}\else\ifnum\pdfstrcmp{#1}{coverageReportsMissing}=0\def\data@out{18.14}\else\ifnum\pdfstrcmp{#1}{earliestOSSProject}=0\def\data@out{2016-10}\else\ifnum\pdfstrcmp{#1}{harnessUpdateStats}=0\let\data@out\data@IX\else\def\data@out{$\PackageError{data}{not found}{use an element}$}\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\data@out}\newcommand\data@V[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\data@V@out{$\PackageError{data}{this is a container: Dict("entriesLow" => 87, "unknown" => 9, "gcovError" => 6, "total" => 322, "intededHarnessRemoval" => 4, "codeChurn" => 28, "projectCode" => 43, "buildFailure" => 27, "libraryCode" => 47, "entriesDecrease" => 71)}{use an element}$}\else\ifnum\pdfstrcmp{#1}{entriesLow}=0\def\data@V@out{$87$}\else\ifnum\pdfstrcmp{#1}{unknown}=0\def\data@V@out{$9$}\else\ifnum\pdfstrcmp{#1}{gcovError}=0\def\data@V@out{$6$}\else\ifnum\pdfstrcmp{#1}{total}=0\def\data@V@out{$322$}\else\ifnum\pdfstrcmp{#1}{intededHarnessRemoval}=0\def\data@V@out{$4$}\else\ifnum\pdfstrcmp{#1}{codeChurn}=0\def\data@V@out{$28$}\else\ifnum\pdfstrcmp{#1}{projectCode}=0\def\data@V@out{$43$}\else\ifnum\pdfstrcmp{#1}{buildFailure}=0\def\data@V@out{$27$}\else\ifnum\pdfstrcmp{#1}{libraryCode}=0\def\data@V@out{$47$}\else\ifnum\pdfstrcmp{#1}{entriesDecrease}=0\def\data@V@out{$71$}\else\def\data@V@out{$\PackageError{data}{not found}{use an element}$}\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\data@V@out}\newcommand\data@IV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\data@IV@out{$\PackageError{data}{this is a container: Dict(:numCommits => 2357857, :numCrashRevisions => 78045, :numIntrospector => 554269, :numHarnessIntrospector => 781749, :numProjects => 342, :numCoverage => 453744, :numHarnessChanges => 9609, :numCves => 1856, :numMonorailBugs => 49020)}{use an element}$}\else\ifnum\pdfstrcmp{#1}{numCommits}=0\def\data@IV@out{$2{,}357{,}857$}\else\ifnum\pdfstrcmp{#1}{numCrashRevisions}=0\def\data@IV@out{$78{,}045$}\else\ifnum\pdfstrcmp{#1}{numIntrospector}=0\def\data@IV@out{$554{,}269$}\else\ifnum\pdfstrcmp{#1}{numHarnessIntrospector}=0\def\data@IV@out{$781{,}749$}\else\ifnum\pdfstrcmp{#1}{numProjects}=0\def\data@IV@out{$342$}\else\ifnum\pdfstrcmp{#1}{numCoverage}=0\def\data@IV@out{$453{,}744$}\else\ifnum\pdfstrcmp{#1}{numHarnessChanges}=0\def\data@IV@out{$9{,}609$}\else\ifnum\pdfstrcmp{#1}{numCves}=0\def\data@IV@out{$1{,}856$}\else\ifnum\pdfstrcmp{#1}{numMonorailBugs}=0\def\data@IV@out{$49{,}020$}\else\def\data@IV@out{$\PackageError{data}{not found}{use an element}$}\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\data@IV@out}\newcommand\data@VI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\data@VI@out{$\PackageError{data}{this is a container: Dict("harnessFail" => 12, "fuzzerRegression" => 4, "revival" => 23, "features" => 29, "other" => 3, "total" => 71)}{use an element}$}\else\ifnum\pdfstrcmp{#1}{harnessFail}=0\def\data@VI@out{$12$}\else\ifnum\pdfstrcmp{#1}{fuzzerRegression}=0\def\data@VI@out{$4$}\else\ifnum\pdfstrcmp{#1}{revival}=0\def\data@VI@out{$23$}\else\ifnum\pdfstrcmp{#1}{features}=0\def\data@VI@out{$29$}\else\ifnum\pdfstrcmp{#1}{other}=0\def\data@VI@out{$3$}\else\ifnum\pdfstrcmp{#1}{total}=0\def\data@VI@out{$71$}\else\def\data@VI@out{$\PackageError{data}{not found}{use an element}$}\fi\fi\fi\fi\fi\fi\fi\data@VI@out}\newcommand\data@VII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\data@VII@out{$\PackageError{data}{this is a container: Dict(:unclean => 491, :removedNotAvailable => 19, :removedClean => 9, :unfiltered => 482)}{use an element}$}\else\ifnum\pdfstrcmp{#1}{unclean}=0\def\data@VII@out{$491$}\else\ifnum\pdfstrcmp{#1}{removedNotAvailable}=0\def\data@VII@out{$19$}\else\ifnum\pdfstrcmp{#1}{removedClean}=0\def\data@VII@out{$9$}\else\ifnum\pdfstrcmp{#1}{unfiltered}=0\def\data@VII@out{$482$}\else\def\data@VII@out{$\PackageError{data}{not found}{use an element}$}\fi\fi\fi\fi\fi\data@VII@out}\newcommand\data@II[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\data@II@out{\PackageError{data}{this is a container: Dict{Symbol, Dict{Symbol, LaTeXStrings.LaTeXString}}(:perProjectRelNoOutliers => Dict(:confIntHigh => L"$0.031$", :estimate => L"$0.023$", :pValue => L"1.1 e^{-12}", :confIntLow => L"$0.015$"), :perProjectRel => Dict(:confIntHigh => L"$0.039$", :estimate => L"$0.028$", :pValue => L"1.0 e^{-14}", :confIntLow => L"$0.019$"), :perProjectCov => Dict(:confIntHigh => L"$0.082$", :estimate => L"$0.03$", :pValue => L"0.21", :confIntLow => L"$-0.018$"), :perProjectCovNoOutliers => Dict(:confIntHigh => L"$0.078$", :estimate => L"$0.028$", :pValue => L"0.22", :confIntLow => L"$-0.018$"), :perHarnessRel => Dict(:confIntHigh => L"$0.017$", :estimate => L"$0.013$", :pValue => L"1.1 e^{-20}", :confIntLow => L"$0.01$"), :perHarnessCovNoOutliers => Dict(:confIntHigh => L"$0.013$", :estimate => L"$0.006$", :pValue => L"0.03", :confIntLow => L"$0.001$"), :perHarnessCov => Dict(:confIntHigh => L"$0.009$", :estimate => L"$0.003$", :pValue => L"0.30", :confIntLow => L"$-0.002$"), :perHarnessRelNoOutliers => Dict(:confIntHigh => L"$0.014$", :estimate => L"$0.01$", :pValue => L"2.7 e^{-17}", :confIntLow => L"$0.007$"))}{use an element}}\else\ifnum\pdfstrcmp{#1}{perProjectRelNoOutliers}=0\let\data@II@out\data@X\else\ifnum\pdfstrcmp{#1}{perProjectRel}=0\let\data@II@out\data@XI\else\ifnum\pdfstrcmp{#1}{perProjectCov}=0\let\data@II@out\data@XII\else\ifnum\pdfstrcmp{#1}{perProjectCovNoOutliers}=0\let\data@II@out\data@XIII\else\ifnum\pdfstrcmp{#1}{perHarnessRel}=0\let\data@II@out\data@XIV\else\ifnum\pdfstrcmp{#1}{perHarnessCovNoOutliers}=0\let\data@II@out\data@XV\else\ifnum\pdfstrcmp{#1}{perHarnessCov}=0\let\data@II@out\data@XVI\else\ifnum\pdfstrcmp{#1}{perHarnessRelNoOutliers}=0\let\data@II@out\data@XVII\else\def\data@II@out{$\PackageError{data}{not found}{use an element}$}\fi\fi\fi\fi\fi\fi\fi\fi\fi\data@II@out}\newcommand\data@XVI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\data@XVI@out{\PackageError{data}{this is a container: Dict{Symbol, LaTeXStrings.LaTeXString}(:confIntHigh => L"$0.009$", :estimate => L"$0.003$", :pValue => L"0.30", :confIntLow => L"$-0.002$")}{use an element}}\else\ifnum\pdfstrcmp{#1}{confIntHigh}=0\def\data@XVI@out{$0.009$}\else\ifnum\pdfstrcmp{#1}{estimate}=0\def\data@XVI@out{$0.003$}\else\ifnum\pdfstrcmp{#1}{pValue}=0\def\data@XVI@out{$0.30$}\else\ifnum\pdfstrcmp{#1}{confIntLow}=0\def\data@XVI@out{$-0.002$}\else\def\data@XVI@out{$\PackageError{data}{not found}{use an element}$}\fi\fi\fi\fi\fi\data@XVI@out}\newcommand\data@XII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\data@XII@out{\PackageError{data}{this is a container: Dict{Symbol, LaTeXStrings.LaTeXString}(:confIntHigh => L"$0.082$", :estimate => L"$0.03$", :pValue => L"0.21", :confIntLow => L"$-0.018$")}{use an element}}\else\ifnum\pdfstrcmp{#1}{confIntHigh}=0\def\data@XII@out{$0.082$}\else\ifnum\pdfstrcmp{#1}{estimate}=0\def\data@XII@out{$0.03$}\else\ifnum\pdfstrcmp{#1}{pValue}=0\def\data@XII@out{$0.21$}\else\ifnum\pdfstrcmp{#1}{confIntLow}=0\def\data@XII@out{$-0.018$}\else\def\data@XII@out{$\PackageError{data}{not found}{use an element}$}\fi\fi\fi\fi\fi\data@XII@out}\newcommand\data@VIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\data@VIII@out{$\PackageError{data}{this is a container: Dict(:numCommits => 8297824, :numCrashRevisions => 104494, :numIntrospector => 975213, :numHarnessIntrospector => 1307652, :numProjects => 510, :numCoverage => 665165, :numHarnessChanges => 42412, :numCves => 3360, :numMonorailBugs => 68486)}{use an element}$}\else\ifnum\pdfstrcmp{#1}{numCommits}=0\def\data@VIII@out{$8{,}297{,}824$}\else\ifnum\pdfstrcmp{#1}{numCrashRevisions}=0\def\data@VIII@out{$104{,}494$}\else\ifnum\pdfstrcmp{#1}{numIntrospector}=0\def\data@VIII@out{$975{,}213$}\else\ifnum\pdfstrcmp{#1}{numHarnessIntrospector}=0\def\data@VIII@out{$1{,}307{,}652$}\else\ifnum\pdfstrcmp{#1}{numProjects}=0\def\data@VIII@out{$510$}\else\ifnum\pdfstrcmp{#1}{numCoverage}=0\def\data@VIII@out{$665{,}165$}\else\ifnum\pdfstrcmp{#1}{numHarnessChanges}=0\def\data@VIII@out{$42{,}412$}\else\ifnum\pdfstrcmp{#1}{numCves}=0\def\data@VIII@out{$3{,}360$}\else\ifnum\pdfstrcmp{#1}{numMonorailBugs}=0\def\data@VIII@out{$68{,}486$}\else\def\data@VIII@out{$\PackageError{data}{not found}{use an element}$}\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\data@VIII@out}\newcommand\data@XVII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\data@XVII@out{\PackageError{data}{this is a container: Dict{Symbol, LaTeXStrings.LaTeXString}(:confIntHigh => L"$0.014$", :estimate => L"$0.01$", :pValue => L"2.7 e^{-17}", :confIntLow => L"$0.007$")}{use an element}}\else\ifnum\pdfstrcmp{#1}{confIntHigh}=0\def\data@XVII@out{$0.014$}\else\ifnum\pdfstrcmp{#1}{estimate}=0\def\data@XVII@out{$0.01$}\else\ifnum\pdfstrcmp{#1}{pValue}=0\def\data@XVII@out{$2.7 e^{-17}$}\else\ifnum\pdfstrcmp{#1}{confIntLow}=0\def\data@XVII@out{$0.007$}\else\def\data@XVII@out{$\PackageError{data}{not found}{use an element}$}\fi\fi\fi\fi\fi\data@XVII@out}\newcommand\data@I[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\data@I@out{$\PackageError{data}{this is a container: Dict(:numCommits => 2556947, :numCrashRevisions => 83863, :numIntrospector => 712094, :numHarnessIntrospector => 929224, :numProjects => 491, :numCoverage => 574840, :numHarnessChanges => 29923, :numCves => 1997, :numMonorailBugs => 53460)}{use an element}$}\else\ifnum\pdfstrcmp{#1}{numCommits}=0\def\data@I@out{$2{,}556{,}947$}\else\ifnum\pdfstrcmp{#1}{numCrashRevisions}=0\def\data@I@out{$83{,}863$}\else\ifnum\pdfstrcmp{#1}{numIntrospector}=0\def\data@I@out{$712{,}094$}\else\ifnum\pdfstrcmp{#1}{numHarnessIntrospector}=0\def\data@I@out{$929{,}224$}\else\ifnum\pdfstrcmp{#1}{numProjects}=0\def\data@I@out{$491$}\else\ifnum\pdfstrcmp{#1}{numCoverage}=0\def\data@I@out{$574{,}840$}\else\ifnum\pdfstrcmp{#1}{numHarnessChanges}=0\def\data@I@out{$29{,}923$}\else\ifnum\pdfstrcmp{#1}{numCves}=0\def\data@I@out{$1{,}997$}\else\ifnum\pdfstrcmp{#1}{numMonorailBugs}=0\def\data@I@out{$53{,}460$}\else\def\data@I@out{$\PackageError{data}{not found}{use an element}$}\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\data@I@out}\newcommand\data@XI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\data@XI@out{\PackageError{data}{this is a container: Dict{Symbol, LaTeXStrings.LaTeXString}(:confIntHigh => L"$0.039$", :estimate => L"$0.028$", :pValue => L"1.0 e^{-14}", :confIntLow => L"$0.019$")}{use an element}}\else\ifnum\pdfstrcmp{#1}{confIntHigh}=0\def\data@XI@out{$0.039$}\else\ifnum\pdfstrcmp{#1}{estimate}=0\def\data@XI@out{$0.028$}\else\ifnum\pdfstrcmp{#1}{pValue}=0\def\data@XI@out{$1.0 e^{-14}$}\else\ifnum\pdfstrcmp{#1}{confIntLow}=0\def\data@XI@out{$0.019$}\else\def\data@XI@out{$\PackageError{data}{not found}{use an element}$}\fi\fi\fi\fi\fi\data@XI@out}\newcommand\data@IX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\data@IX@out{$\PackageError{data}{this is a container: Dict{Symbol, Real}(:max => 93.0, :min => -85.98, :deviation => 4.48, :mean => 0.25, :count => 6520, :median => 0.0)}{use an element}$}\else\ifnum\pdfstrcmp{#1}{max}=0\def\data@IX@out{$93.0$}\else\ifnum\pdfstrcmp{#1}{min}=0\def\data@IX@out{$-85.98$}\else\ifnum\pdfstrcmp{#1}{deviation}=0\def\data@IX@out{$4.48$}\else\ifnum\pdfstrcmp{#1}{mean}=0\def\data@IX@out{$0.25$}\else\ifnum\pdfstrcmp{#1}{count}=0\def\data@IX@out{$6{,}520$}\else\ifnum\pdfstrcmp{#1}{median}=0\def\data@IX@out{$0.0$}\else\def\data@IX@out{$\PackageError{data}{not found}{use an element}$}\fi\fi\fi\fi\fi\fi\fi\data@IX@out}\newcommand\data@XIV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\data@XIV@out{\PackageError{data}{this is a container: Dict{Symbol, LaTeXStrings.LaTeXString}(:confIntHigh => L"$0.017$", :estimate => L"$0.013$", :pValue => L"1.1 e^{-20}", :confIntLow => L"$0.01$")}{use an element}}\else\ifnum\pdfstrcmp{#1}{confIntHigh}=0\def\data@XIV@out{$0.017$}\else\ifnum\pdfstrcmp{#1}{estimate}=0\def\data@XIV@out{$0.013$}\else\ifnum\pdfstrcmp{#1}{pValue}=0\def\data@XIV@out{$1.1 e^{-20}$}\else\ifnum\pdfstrcmp{#1}{confIntLow}=0\def\data@XIV@out{$0.01$}\else\def\data@XIV@out{$\PackageError{data}{not found}{use an element}$}\fi\fi\fi\fi\fi\data@XIV@out}\newcommand\data@III[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\data@III@out{\PackageError{data}{this is a container: Dict{Symbol, Dict{Symbol, LaTeXStrings.LaTeXString}}(:bugs => Dict(:estimate => L"$0.649$", :pValue => L"2.2 e^{-16}"), :cov => Dict(:estimate => L"$-0.365$", :pValue => L"4.2 e^{-12}"))}{use an element}}\else\ifnum\pdfstrcmp{#1}{bugs}=0\let\data@III@out\data@XVIII\else\ifnum\pdfstrcmp{#1}{cov}=0\let\data@III@out\data@XIX\else\def\data@III@out{$\PackageError{data}{not found}{use an element}$}\fi\fi\fi\data@III@out}\newcommand\data@XIX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\data@XIX@out{\PackageError{data}{this is a container: Dict{Symbol, LaTeXStrings.LaTeXString}(:estimate => L"$-0.365$", :pValue => L"4.2 e^{-12}")}{use an element}}\else\ifnum\pdfstrcmp{#1}{estimate}=0\def\data@XIX@out{$-0.365$}\else\ifnum\pdfstrcmp{#1}{pValue}=0\def\data@XIX@out{$4.2 e^{-12}$}\else\def\data@XIX@out{$\PackageError{data}{not found}{use an element}$}\fi\fi\fi\data@XIX@out}\newcommand\data@XIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\data@XIII@out{\PackageError{data}{this is a container: Dict{Symbol, LaTeXStrings.LaTeXString}(:confIntHigh => L"$0.078$", :estimate => L"$0.028$", :pValue => L"0.22", :confIntLow => L"$-0.018$")}{use an element}}\else\ifnum\pdfstrcmp{#1}{confIntHigh}=0\def\data@XIII@out{$0.078$}\else\ifnum\pdfstrcmp{#1}{estimate}=0\def\data@XIII@out{$0.028$}\else\ifnum\pdfstrcmp{#1}{pValue}=0\def\data@XIII@out{$0.22$}\else\ifnum\pdfstrcmp{#1}{confIntLow}=0\def\data@XIII@out{$-0.018$}\else\def\data@XIII@out{$\PackageError{data}{not found}{use an element}$}\fi\fi\fi\fi\fi\data@XIII@out}\newcommand\data@XV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\data@XV@out{\PackageError{data}{this is a container: Dict{Symbol, LaTeXStrings.LaTeXString}(:confIntHigh => L"$0.013$", :estimate => L"$0.006$", :pValue => L"0.03", :confIntLow => L"$0.001$")}{use an element}}\else\ifnum\pdfstrcmp{#1}{confIntHigh}=0\def\data@XV@out{$0.013$}\else\ifnum\pdfstrcmp{#1}{estimate}=0\def\data@XV@out{$0.006$}\else\ifnum\pdfstrcmp{#1}{pValue}=0\def\data@XV@out{$0.03$}\else\ifnum\pdfstrcmp{#1}{confIntLow}=0\def\data@XV@out{$0.001$}\else\def\data@XV@out{$\PackageError{data}{not found}{use an element}$}\fi\fi\fi\fi\fi\data@XV@out}\newcommand\data@X[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\data@X@out{\PackageError{data}{this is a container: Dict{Symbol, LaTeXStrings.LaTeXString}(:confIntHigh => L"$0.031$", :estimate => L"$0.023$", :pValue => L"1.1 e^{-12}", :confIntLow => L"$0.015$")}{use an element}}\else\ifnum\pdfstrcmp{#1}{confIntHigh}=0\def\data@X@out{$0.031$}\else\ifnum\pdfstrcmp{#1}{estimate}=0\def\data@X@out{$0.023$}\else\ifnum\pdfstrcmp{#1}{pValue}=0\def\data@X@out{$1.1 e^{-12}$}\else\ifnum\pdfstrcmp{#1}{confIntLow}=0\def\data@X@out{$0.015$}\else\def\data@X@out{$\PackageError{data}{not found}{use an element}$}\fi\fi\fi\fi\fi\data@X@out}\newcommand\data@XVIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\data@XVIII@out{\PackageError{data}{this is a container: Dict{Symbol, LaTeXStrings.LaTeXString}(:estimate => L"$0.649$", :pValue => L"2.2 e^{-16}")}{use an element}}\else\ifnum\pdfstrcmp{#1}{estimate}=0\def\data@XVIII@out{$0.649$}\else\ifnum\pdfstrcmp{#1}{pValue}=0\def\data@XVIII@out{$2.2 e^{-16}$}\else\def\data@XVIII@out{$\PackageError{data}{not found}{use an element}$}\fi\fi\fi\data@XVIII@out}\makeatother

